Sharp asymptotic and finite-sample rates of convergence of empirical measures in Wasserstein distance

The Wasserstein distance between two probability measures on a metric space is a measure of closeness with applications in statistics, probability, and machine learning. In this work, we consider the fundamental question of how quickly the empirical measure obtained from $n$ independent samples from $\mu$ approaches $\mu$ in the Wasserstein distance of any order. We prove sharp asymptotic and finite-sample results for this rate of convergence for general measures on general compact metric spaces. Our finite-sample results show the existence of multi-scale behavior, where measures can exhibit radically different rates of convergence as $n$ grows.

==> commands.tex <==

\usepackage{amsmath, amssymb, color}
\usepackage{amsthm} 
%\usepackage{natbib}
\usepackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
\usepackage{xcolor,colortbl}
%
\RequirePackage{hypernat}
\usepackage{cleveref}
%
\usepackage{color}
\usepackage{amsfonts, fancybox}
\usepackage{amssymb}
\usepackage[american]{babel}
% \addto{\captionsamerican}{\renewcommand{\abstractname}{}}
%
\usepackage{psfrag,color}
\usepackage{dcolumn}
% \usepackage{subfigure}
\usepackage[format=hang, justification=justified, singlelinecheck=false]{subcaption}
\usepackage{flafter, bm, dsfont}
\usepackage[section]{placeins}
\usepackage[final]{showkeys}
\renewcommand*\showkeyslabelformat[1]{%
\fbox{\normalfont\tiny\ttfamily#1}}


\usepackage{multirow}
\usepackage{color}
\usepackage{amsmath}
\usepackage{float}
\usepackage{mathrsfs}
\usepackage{amsfonts}
\usepackage{dsfont}
\usepackage{amssymb}
%
%\usepackage{algorithmic, algorithm}
\usepackage{wrapfig}


\usepackage{amssymb, latexsym}

%
\usepackage{graphicx}
%
\usepackage{epstopdf}
\usepackage{tikz}
\usepackage{pgfplots}
\usepgfplotslibrary{fillbetween}

%% if you need to pass options to natbib, use, e.g.:
%% \PassOptionsToPackage{numbers, compress}{natbib}
%% before loading nips_2017
%%
%% to avoid loading the natbib package, add option nonatbib:
%%\usepackage[nonatbib]{nips_2017}
%
%%\usepackage[nonatbib]{nips_2017}
%
%% to compile a camera-ready version, replace the above line with the following, which has the [final] option, e.g.:
%% \usepackage[final]{nips_2017}
%
%\usepackage[utf8]{inputenc} % allow utf-8 input
%\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
%\usepackage{hyperref}       % hyperlinks
%\usepackage{url}            % simple URL typesetting
%\usepackage{booktabs}       % professional-quality tables
%\usepackage{amsfonts}       % blackboard math symbols
%\usepackage{nicefrac}       % compact symbols for 1/2, etc.
%\usepackage{microtype}      % microtypography
%\usepackage{wrapfig}        % for wrapping figures
%\usepackage[notref, notcite, final]{showkeys}
%
%\usepackage{amsmath, amsthm, amsfonts}
%\usepackage{dsfont}
%\usepackage[sort]{cite}
%\usepackage{graphicx}
%
%% Notes
\usepackage{color}
\newcommand{\jw}[1]{{\textcolor{red}{[\textbf{JON:} #1]}}}
%\newcommand{\pr}[1]{{\textcolor{blue}{[\textbf{PR:} #1]}}}
%
%% For algorithms
\usepackage{algorithm}
%%\usepackage[noend]{algorithmic}
\usepackage[noend]{algcompatible}
%
%% Theorem definitions
\newtheorem{definition}{Definition}%[section]
\newtheorem{theorem}{Theorem}%[section]
\newtheorem{exe}{Exercise}%[section]
\newtheorem{exa}{Example}%[section]
\newtheorem{fact}{Fact}%[section]
\newtheorem{proposition}{Proposition}%[section]
\newtheorem{lemma}{Lemma}%[section]
\newtheorem{corollary}{Corollary}%[thm]
\newtheorem{conj}{Conjecture}%[section]
\newtheorem{remark}{Remark}%[section]
\newtheorem{discussion}{Discussion}%[section]
\newtheorem{conc}{Conclusion}%[section]

% Custom definitions

\newcommand{\cA}{\mathcal{A}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cI}{\mathcal{I}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cQ}{\mathcal{Q}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cY}{\mathcal{Y}}
\newcommand{\cZ}{\mathcal{Z}}

\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bD}{\mathbf{D}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bH}{\mathbf{H}}
\newcommand{\bI}{\mathbf{I}}
\newcommand{\bJ}{\mathbf{J}}
\newcommand{\bK}{\mathbf{K}}
\newcommand{\bM}{\mathbf{M}}
\newcommand{\bN}{\mathbf{N}}
\newcommand{\bO}{\mathbf{O}}
\newcommand{\bP}{\mathbf{P}}
\newcommand{\bQ}{\mathbf{Q}}
\newcommand{\bS}{\mathbf{S}}
\newcommand{\bT}{\mathbf{T}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bV}{\mathbf{V}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}}


%\renewcommand{\subseteq}{\subset}

\newcommand{\R}{{\rm I}\kern-0.18em{\rm R}}
\newcommand{\h}{{\rm I}\kern-0.18em{\rm H}}
\newcommand{\PP}{{\rm I}\kern-0.18em{\rm P}}
\newcommand{\E}{{\rm I}\kern-0.18em{\rm E}}
\newcommand{\Z}{{\rm Z}\kern-0.18em{\rm Z}}
\newcommand{\1}{{\rm 1}\kern-0.24em{\rm I}}
\newcommand{\N}{{\rm I}\kern-0.18em{\rm N}}

\newcommand{\DS}{\displaystyle}
\DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmin}{argmin}
\newcommand{\Tr}{\mathrm{Tr}}
\newcommand{\eps}{\varepsilon}
\newcommand{\del}{\delta}
\newcommand{\re}{\R}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\plusminus}{\raisebox{.2ex}{$\scriptstyle\pm$}}
\newcommand{\nnz}{\text{nnz}}
%\DeclareMathOperator*{\KL}{D_{\mathrm{KL}}}
\newcommand{\KL}{\cK}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\diag}{\mathbf{D}}
\newcommand{\ones}{\bone_n}
\newcommand{\tildo}{\widetilde{O}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\bone}{\mathbf{1}}

\newcommand{\errr}{\text{err}_r}
\newcommand{\errrp}{\text{err}_r^{(+)}}
\newcommand{\errrn}{\text{err}_r^{(-)}}
\newcommand{\errc}{\text{err}_c}
\newcommand{\errcp}{\text{err}_c^{(+)}}
\newcommand{\errcn}{\text{err}_c^{(-)}}
\newcommand{\Cinfty}{\|C\|_{\infty}}

\newcommand{\zeroesr}{\text{zeroes}_r}
\newcommand{\zeroesc}{\text{zeroes}_c}

\newcommand{\Pavg}{P_{\text{avg}}}
\newcommand{\Pavgex}{P_{\text{avg}}^{\text{exact}}}
\newcommand{\Ptex}{P_t^{\text{exact}}}
\newcommand{\Pbar}{{\bar{P}}}
\newcommand{\Pprime}{P'}
\newcommand{\Pex}{Q^{\text{sink}}}
\newcommand{\Qsink}{\Pex}
\newcommand{\Poptprime}{(P^*)'}

\newcommand{\U}{\cU_{r,c}}
\newcommand{\Ubar}{\cU_{\rbar, \cbar}}
\newcommand{\Uprime}{\cU_{r', c'}}
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\Peta}{P_\eta}
\newcommand{\sink}{\Pi_{\cS}}

% algorithm names (feel free to change these!)
\newcommand{\lmdot}{\textsc{lmdot}}
\newcommand{\ot}{\textsc{ApproxOT}}
\newcommand{\lmd}{\textsc{lmd}}
\newcommand{\roundtrans}{\textsc{round}}
\newcommand{\approxsink}{\textsc{approxsinkhorn}}
\newcommand{\sinkhorn}{\textsc{Sinkhorn}}
\newcommand{\threshold}[1]{\textsc{threshold}_{#1}}
\newcommand{\approxproj}{\textsc{Proj}}
\newcommand{\greedy}{\textsc{Greenkhorn}}

